Decomposition, Reformulation, and Diving in University Course Timetabling

In many real-life optimisation problems, there are multiple interacting components in a solution. For example, different components might specify assignments to different kinds of resource. Often, each component is associated with different sets of soft constraints, and so with different measures of soft constraint violation. The goal is then to minimise a linear combination of such measures. This paper studies an approach to such problems, which can be thought of as multiphase exploitation of multiple objective-/value-restricted submodels. In this approach, only one computationally difficult component of a problem and the associated subset of objectives is considered at first. This produces partial solutions, which define interesting neighbourhoods in the search space of the complete problem. Often, it is possible to pick the initial component so that variable aggregation can be performed at the first stage, and the neighbourhoods to be explored next are guaranteed to contain feasible solutions. Using integer programming, it is then easy to implement heuristics producing solutions with bounds on their quality. Our study is performed on a university course timetabling problem used in the 2007 International Timetabling Competition, also known as the Udine Course Timetabling Problem. In the proposed heuristic, an objective-restricted neighbourhood generator produces assignments of periods to events, with decreasing numbers of violations of two period-related soft constraints. Those are relaxed into assignments of events to days, which define neighbourhoods that are easier to search with respect to all four soft constraints. Integer programming formulations for all subproblems are given and evaluated using ILOG CPLEX 11. The wider applicability of this approach is analysed and discussed.

==> implementation.tex <==
\section{The Implementation}
\label{sec:implement}

The proposed heuristic has been implemented using ILOG Concert libraries in C++ \citep{cplex10apt}.
ILOG CPLEX 10 is used both at \textbf{Surface} and in all dives.
Other features of the implementation seem to bring about only modest improvements 
 in terms of performance:
\begin{itemize}
\item Thanks to the presence of set $\Deprecated$ of forbidden course-period allocations
 in the input to the problem, little symmetry seems to remain and further symmetry-breaking seems of little use 
\item Design of cutting planes and related separation routines surpassing stand-alone 
 CPLEX seems to be non-trivial in the case of graph colouring \citep{MendezDiaz2008},
 and certainly is difficult for problems with a graph-colouring component, where
 the objective is to minimise the number of violations of non-trivial soft constraints \citep{Avella2005}.
The few standard cuts for the decision version of the graph colouring component \citep{MendezDiaz2008},
 perhaps some from bipartite matching \cite{Gwan1992,Balas1993},
 and several problem-specific cuts from implied bounds seem to be the best one can hope for.
Our implementation also uses cuts from enumeration of patterns, introduced by \cite{Marecek2007GOR}.
\item Considering the auto-tuning capabilities of CPLEX 10, attempts to hand-craft 
 parameter settings seem almost futile.
\end{itemize} 
We have, however, tried to come up with a robust implementation, performing well across
 all instances from the International Timetabling Competition 2007. 

\subsection{Cuts from Cliques}

The graph colouring formulation we use is known to be rather weak \citep{Caprara1998}.
\citet{Chvatal2006} has shown it can be strengthened to the point of being a convex 
hull of integer points using valid inequalities from cliques. In timetabling terms, 
these corresponds to collection $\Cliques$ of sets of courses, which correspond to
complete subgraphs in the course-based conflict graph.
Hence at \textbf{Surface}, we can add: 
\begin{align}
  \label{eqn:cliquecuts}
  \hskip 2cm \forall q \in \Cliques \forall p \in \Periods \hskip 2cm & \sum_{c \in q} & \SetTimes{p,c} & \le 1
\end{align} 
The number of valid inequalities one can obtain from cliques, however, 
is the product of the upper bound on the number of colours and the number of cliques
in the graph, which is exponential. Moreover, generating large cliques, which are most 
useful, is obviously hard for any heuristic, both in theory \citep{Zuckerman2007} 
and in practice \citep{MendezDiaz2008}. We are hence using two imperfect separation 
routines to add only violated valid inequalities (cuts) at individual nodes. 
In the first routine, we check for violations of a small number of large cliques, 
discovered at the root node. (That is within the reported time limit.)
In the second routine, we check for violations of triangles. If we find a triangle
that violates the inequality (\ref{eqn:cliquecuts}), we try to ``grow'' it into a large clique.
If this ``growing'' makes any progress, we use the cut from the resulting larger clique.
Otherwise, we discard the cut.
In both the large clique discovery and enumeration of triangles, we benefit greatly
from using a course-based conflict graph \citep{Marecek2007TR}, which is much
smaller than the event-based one. 

\subsection{Cuts from Implied Bounds}

\citet{Marecek2008TR} describe eight classes of constraints derived from ``implied bounds''. 
In the present version of the solver, we have added two of these constraints statically 
to the formulation of diving, with the rather surprising effect of halving the run-times 
of CPLEX Barrier LP solver for the relaxation. Those constraints were:

\begin{align}
\hskip 2cm \forall c \in \Courses \hskip 2cm & \sum_{d \in \Days} \CourseSchedule{d,c} & \ge 1 \\
\hskip 2cm \forall c \in \Courses \hskip 2cm & \sum_{r \in \Rooms} \CourseRooms{r,c} & \ge 1 
\end{align}

\subsection{Cuts from Event/Free-Period Patterns}

Further improvements in performance can be gained by strengthening the ``natural'' 
 penalising patterns constraints (\ref{eqn:ng:patmat1}--\ref{eqn:ng:patmat4})
 by enumeration of daily patterns and the penalties they incur \citep{Marecek2007TR}. 
When $n$ is the number of periods per day,
patterns in timetables of individual curricula can also be thought of as $A = \left\langle {a_1, \ldots, a_n} \right\rangle$, 
where $a_i$ is equal to one if there is an event in the timetable of the given curriculum in 
period $i$ of the given day and $-1$ otherwise.  
In a problem instance with four periods per day, penalisation of the pattern $A = \left\langle {a_1, a_2, a_3, a_4} \right\rangle$
with penalty $p$ and $m = \sum_{a \in A, a = 1} a$ can be formulated as:
\begin{multline}
  \label{eqn:ng:patmatSchema}
   \forall u \in \Curricula \; \forall d \in \Days \; \forall \left\langle {p_1, p_2, p_3, p_4} \right\rangle \in \HasPeriods{d} \\
  p \; ( a_1  \sum_{c \in \CurriculumHasCourses{u}} \SetTimes{c,p_1}  
      +  a_2  \sum_{c \in \CurriculumHasCourses{u}} \SetTimes{c,p_2}
      +  a_3  \sum_{c \in \CurriculumHasCourses{u}} \SetTimes{c,p_3} 
       + a_4  \sum_{c \in \CurriculumHasCourses{u}} \SetTimes{c,p_4} - m) \\ 
  \le \sum_{s \in \SingletonChecks} \Singletons{u,d,s}
\end{multline}

\subsection{Further Details}

Finally, a limited experimentation with ``manual'' tuning of parameters has been 
 attempted on the instances from the International Timetabling Competition 2007. 
Except for the very first dive per run, the best previously found upper bound for the
 complete problem is also injected into all dives as an upper cut-off point.
\textbf{PeriodFixed} dives are always run before \textbf{DayFixed} dives, both
 with a strict time limit.  
Additionally, we also use the following CPLEX settings:
\begin{itemize}
\item CPLEX Barrier LP solver is used at the root node, both at \textbf{Surface} and in all dives
\item In all dives, CPLEX emphasis is set to ``integer feasibility''
      and ``aggressive symmetry breaking'' , with ``very aggressive''
      generation of fractional cuts enabled
%\item Branching direction is always up first and minimum objective difference is set to one
%\item The minimum objective difference is set to one
\item Each \textbf{PeriodFixed} dive is running until the time limit of 180 seconds has been 
 exhausted or until a solution within 2 \% of the lower bound has been obtained, 
 whichever comes first
\item Each \textbf{DayFixed} dive is running until the time limit of 15 minutes has been 
 exhausted or until a solution within 2 \% of the lower bound has been obtained, 
 whichever comes first. 
\end{itemize}
Outside of the choice of the method of linear programming, however,  
 the default settings and auto-tuning procedures of CPLEX seem to perform 
 reasonably well.

\TODO{try again objective difference set to 10!}
\TODO{RINS heuristics every 100 nodes, and clique cut generation has been turned to aggressive?}

